Precise determination of $\alpha_{S}(M_Z)$ from a global fit of energy-energy correlation to NNLO+NNLL predictions

We present a comparison of the computation of energy-energy correlation in $e^{+}e^{-}$ collisions in the back-to-back region at next-to-next-to-leading logarithmic accuracy matched with the next-to-next-to-leading order perturbative prediction to LEP, PEP, PETRA, SLC and TRISTAN data. With these predictions we perform an extraction of the strong coupling constant taking into account non-perturbative effects modelled with Monte Carlo event generators. The final result at NNLO+NNLL precision is $\alpha_{S}(M_{Z})=0.11750\pm 0.00018 {\text( exp.)}\pm 0.00102{\text(hadr.)}\pm0.00257{\text(ren.)}\pm 0.00078{\text(res.)}$.

==> Makefile <==
#ulimit -u 10000
latexfile=EECALPHAS
newname?=EECALPHAS
STYLE=arxiv

#LATEX=  lualatex -halt-on-error -shell-escape -enable-write18
LATEX=  lualatex -halt-on-error -shell-escape -enable-write18
BIBTEX=bibtex


ifeq ($(STYLE),draft)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-draft.tex 
endif

ifeq ($(STYLE),arxiv)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-arxiv.tex 
endif

ifeq ($(STYLE),epjc)
	STYLE_SPECIFIC_FILES=svjour.cls  svepj.clo $(latexfile)-epjc.tex
endif


all: $(latexfile)-$(STYLE).pdf

tar:  Makefile $(figures) fitranges.tex $(latexfile)-val.tex $(latexfile)-def.tex $(constanttables) $(tables) $(latexfile).bst $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex $(latexfile)-ank.tex $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	mkdir -p TAR/Figures
#	mkdir -p TAR/Tables
#	mkdir -p TAR/ConstantTables
	cp Makefile   fitranges.tex $(latexfile).bst $(latexfile).bib $(latexfile)-val.tex $(latexfile)-def.tex $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex  $(latexfile)-ank.tex  $(STYLE_SPECIFIC_FILES) TAR
#	cp $(constanttables) TAR/ConstantTables
#	cp $(tables) TAR/Tables
	cp $(figures) TAR/Figures
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/*tex	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	sed -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	sed -i '/@artic/achecked={2},'     TAR/*bib	
	sed -i '/@inproceed/achecked={2},' TAR/*bib	
	sed -i '/@phdthesis/achecked={2},' TAR/*bib	

ifeq ($(STYLE),epjc)
	sed -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
	sed -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
endif
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
	mv TAR/$(latexfile)-txt.tex TAR/$(newname)-txt.tex
	mv TAR/$(latexfile)-val.tex TAR/$(newname)-val.tex
	mv TAR/$(latexfile)-def.tex TAR/$(newname)-def.tex
	mv TAR/$(latexfile)-ank.tex TAR/$(newname)-ank.tex
	mv TAR/$(latexfile)-abs.tex TAR/$(newname)-abs.tex
	mv TAR/$(latexfile)-tab.tex TAR/$(newname)-tab.tex
	mv TAR/$(latexfile)-fig.tex TAR/$(newname)-fig.tex
ifeq ($(STYLE),arxiv)
       #####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
	tar -zcvf   $(newname).tar.gz -C TAR . 
	rm -rf TAR

#cat EECALPHAS-txt.tex  | grep -oh "\w*-figure0\.pdf\w*"* | sort | uniq
figures=Figures/figcorrJADE2-figure0.pdf \
Figures/figcorrOPAL-figure0.pdf \
Figures/figcorrTOPAZ-figure0.pdf \
Figures/figdependencebmass-figure0.pdf \
Figures/figdependencehadr-figure0.pdf \
Figures/figdependencepower-figure0.pdf \
Figures/figdependencescalerenorm-figure0.pdf \
Figures/figdependencescaleresum-figure0.pdf \
Figures/figdependencesqrtsC-figure0.pdf \
Figures/figdependencesqrtsL-figure0.pdf \
Figures/figdependencesqrtsM-figure0.pdf \
Figures/figdependencesqrtsrangetwo5-figure0.pdf \
Figures/fighadrrewJADE2-figure0.pdf \
Figures/fighadrrewJADE3-figure0.pdf \
Figures/fighadrrewJADE-figure0.pdf \
Figures/fighadrrewMAC-figure0.pdf \
Figures/fighadrrewOPAL-figure0.pdf \
Figures/fighadrrewTASSO4-figure0.pdf \
Figures/fighadrrewTOPAZ2-figure0.pdf \
Figures/fighadrrewTOPAZ-figure0.pdf \
Figures/figmcherwigrewJADE2-figure0.pdf \
Figures/figmcherwigrewJADE3-figure0.pdf \
Figures/figmcherwigrewJADE-figure0.pdf \
Figures/figmcherwigrewMAC-figure0.pdf \
Figures/figmcherwigrewOPAL-figure0.pdf \
Figures/figmcherwigrewTASSO4-figure0.pdf \
Figures/figmcherwigrewTOPAZ2-figure0.pdf \
Figures/figmcherwigrewTOPAZ-figure0.pdf \
Figures/figmcsherparewJADE2-figure0.pdf \
Figures/figmcsherparewJADE3-figure0.pdf \
Figures/figmcsherparewJADE-figure0.pdf \
Figures/figmcsherparewMAC-figure0.pdf \
Figures/figmcsherparewOPAL-figure0.pdf \
Figures/figmcsherparewTASSO4-figure0.pdf \
Figures/figmcsherparewTOPAZ2-figure0.pdf \
Figures/figmcsherparewTOPAZ-figure0.pdf \
Figures/figresultCELLO2-figure0.pdf \
Figures/figresultCELLO-figure0.pdf \
Figures/figresultDELPHI-figure0.pdf \
Figures/figresultJADE2-figure0.pdf \
Figures/figresultJADE3-figure0.pdf \
Figures/figresultJADE-figure0.pdf \
Figures/figresultL3-figure0.pdf \
Figures/figresultMAC-figure0.pdf \
Figures/figresultMARKII2-figure0.pdf \
Figures/figresultMARKII-figure0.pdf \
Figures/figresultOPAL3-figure0.pdf \
Figures/figresultOPAL-figure0.pdf \
Figures/figresultPLUTO-figure0.pdf \
Figures/figresultSLD-figure0.pdf \
Figures/figresultTASSO2-figure0.pdf \
Figures/figresultTASSO3-figure0.pdf \
Figures/figresultTASSO4-figure0.pdf \
Figures/figresultTASSO-figure0.pdf \
Figures/figresultTOPAZ2-figure0.pdf \
Figures/figresultTOPAZ-figure0.pdf \
Figures/ruler-figure0.pdf 
tables=
constanttables=


$(latexfile)-$(STYLE).pdf :  $(figures) $(constanttables) $(tables) $(latexfile).bst\
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                     $(latexfile)-fig.tex $(latexfile)-ank.tex   $(STYLE_SPECIFIC_FILES)
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)

#$(latexfile).pdf : $(latexfile).ps
#	ps2pdf -dUseCIEColor -dPDFSETTINGS=/printer -sPAPERSIZE=a4  $(latexfile).ps $(latexfile).pdf

#ps : $(latexfile)-$(STYLE).ps 

pdf : $(latexfile)-$(STYLE).pdf
#$(latexfile).ps : $(latexfile).dvi
#	dvips -Ppdf -t a4 $(latexfile)


$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
		for a in $$(ls -1 $(latexfile)-*.tex | grep -v auth | grep -v ank ); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws --add-tex-command="Cref p" --add-tex-command="refr p" --add-tex-command="Refrs p" \
		--add-tex-command="Refr p" --add-tex-command="eqn p" --add-tex-command="eqns pp" --add-tex-command="eqnss pp"         -t --dont-tex-check-comments -d en_GB -c $$a ;\
		done

clean :
	rm -f $(latexfile)-papers.tex
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm

pics:
	mkdir -p Figures
	mkdir -p Figures/plots_results/eps
	mkdir -p Figures/plots_energy_results/eps
	cp -r ../../output/plots_results/eps/* Figures/plots_results/eps/
	cp -r ../../output/plots_energy_results/eps/* Figures/plots_energy_results/eps/


